A Stochastic Approach to Classification Error Estimates in Convolutional Neural Networks

This technical report presents research results achieved in the field of verification of trained Convolutional Neural Network (CNN) used for image classification in safety-critical applications. As running example, we use the obstacle detection function needed in future autonomous freight trains with Grade of Automation (GoA) 4. It is shown that systems like GoA 4 freight trains are indeed certifiable today with new standards like ANSI/UL 4600 and ISO 21448 used in addition to the long-existing standards EN 50128 and EN 50129. Moreover, we present a quantitative analysis of the system-level hazard rate to be expected from an obstacle detection function. It is shown that using sensor/perceptor fusion, the fused detection system can meet the tolerable hazard rate deemed to be acceptable for the safety integrity level to be applied (SIL-3). A mathematical analysis of CNN models is performed which results in the identification of classification clusters and equivalence classes partitioning the image input space of the CNN. These clusters and classes are used to introduce a novel statistical testing method for determining the residual error probability of a trained CNN and an associated upper confidence limit. We argue that this greybox approach to CNN verification, taking into account the CNN model's internal structure, is essential for justifying that the statistical tests have covered the trained CNN with its neurons and inter-layer mappings in a comprehensive way.

==> glossary.tex <==

% =======================================================================
\newglossaryentry{Accident} {
	name=Accident,
	text=accident,
	description={An unexpected event that causes damage, injury, or harm. See also  \gls{Incident}}
}

\newglossaryentry{Adaptivity} {
	name=Adaptivity,
	description={The ability to improve performance by learning from experience. [In the Machine Learning context], a system is considered adaptive when it continues to learn in real-time operation}
}

\newglossaryentry{Artificial intelligence (AI)} {
	name={Artificial intelligence (AI)},
	text={artificial intelligence (AI)},
	description={Technology that appears to emulate human performance typically by learning, coming to its own conclusions, appearing to understand complex content, engaging in natural dialogues with people, enhancing human cognitive performance (also known as cognitive computing) or replacing people on execution of non-routine tasks. Applications include autonomous vehicles, automatic speech recognition and generation, and detection of novel concepts and abstractions (useful for detecting potential new risks and aiding humans to quickly understand very large bodies of ever-changing information)}
}
  
\newglossaryentry{Neural network} {
	name={Neural network},
	text={neural network},
	description={A computational graph that consists of connected nodes (‘neurons’) that define the order in which operations are performed on the input. Neurons are connected by edges, which are parameterised by weights (and biases). Neurons are organised in layers, specifically an input layer, several intermediate layers, and an output layer. This document refers to a specific type of neural network that is particularly suited to process image data: convolutional neural networks (CNNs) which use parameterised convolution operations to compute their outputs. Commonly used types of neural networks are to be highlighted:  \gls{Convolutional neural networks (CNNs)}, \gls{Recurrent neural networks (RNNs)}, \gls{Generative adversarial networks (GANs)} }
}

\newglossaryentry{Artificial neural network (ANN)} {
	name={Artificial neural network (ANN)},
	text={Artificial neural network},
	description={A computational graph that consists of connected nodes (‘neurons’) that define the order in which operations are performed on the input. Neurons are connected by edges, which are parameterised by weights (and biases). Neurons are organised in layers, specifically an input layer, several intermediate layers, and an output layer. This document refers to a specific type of neural network that is particularly suited to process image data: convolutional neural networks (CNNs) which use parameterised convolution operations to compute their outputs. Commonly used types of neural networks are to be highlighted:  \gls{Convolutional neural networks (CNNs)}, \gls{Recurrent neural networks (RNNs)}, \gls{Generative adversarial networks (GANs)} }
}

\newglossaryentry {Convolutional neural networks (CNNs)} {
	name= {Convolutional neural networks (CNNs)},
	description={ - a specialised kind of neural network for processing data that has a known grid-like topology. Convolutional networks use convolution [a specialised kind of linear operation] in place of general matrix multiplication in at least one of their layers}
}

\newglossaryentry  {Recurrent neural networks (RNNs)} {
	name={Recurrent neural networks (RNNs)},
	description={- a type of advanced artificial neural network (ANN) that involves directed cycles in memory. One aspect of recurrent neural networks is the ability to build on earlier types of networks with fixed-size input vectors and output vectors}
}

\newglossaryentry {Generative adversarial networks (GANs)} {
	name={Generative adversarial networks (GANs)},
	description={- a type of construct in neural network technology that is composed of two neural networks: a generative network and a discriminative network. These work together to provide high-level simulation of conceptual tasks}
}

\newglossaryentry{Automation} {
	name=Automation,
	text=automation,
	description={The use of control systems and information technologies reducing the need for human [input]11 , typically for repetitive tasks}
}

\newglossaryentry{Autonomy} {
	name=Autonomy,
	text=autonomy,
	description={The ability to perform tasks in complex environments without input by a human}
}

\newglossaryentry{Avionics} {
	name=Avionics,
	text=avionics,
	description={Electronics (including computers), as applied in aviation}
} 

\newglossaryentry{Bias} {
	name=Bias,
	text=bias,
	description={An error from erroneous assumptions in the learning [process]. High bias can cause an algorithm to miss the relevant relations between attributes and target outputs (=underfitting)}
}

\newglossaryentry{Big Data} {
	name={Big Data},
	description={A new technology, which allows the analysis of big amount of data (more than terabytes), with a high velocity (high speed of data processing), from various sources (sensors, images, texts, etc.), and which might be unstructured (not standardised format)}
}

\newglossaryentry{Brittle} {
	name={Brittle (deep neural network)},
	text=brittle,
	description={A trained DNN is called brittle if seemingly small changes in  the input data lead to drastic changes in the output, resulting, for example, in an erroneous image classification}
}

\newglossaryentry{cloud-native repository} {
	name={cloud-native repository},
	description={A data archive residing in the cloud which can be evaluated and manipulated in the cloud as well, without the necessity to download this data to local computers}
}

\newglossaryentry{DARPA} {
	name={DARPA (Defence Advanced Research Projects Agency)},
	description={A US Government Agency whose mission is to make pivotal investments in breakthrough technologies for national security}
}

\newglossaryentry{Data-driven AI} {
	name={Data-driven AI},
	description={The data-driven [approach] focuses on building a system that can [learn] what is the right answer based on having [trained on] a large number of [labelled] examples}
}

\newglossaryentry{Data science} {
	name={Data science},
	description={A broad field that refers to the collective processes, theories, concepts, tools and technologies that enable the review, analysis and extraction of valuable knowledge and information from raw data}
}

\newglossaryentry{Data for safety (EASA)} {
	name={Data for safety (EASA)},
	description={
		Data4Safety (also known as D4S) is a data collection and analysis programme that supports the goal of ensuring the highest common level of safety and environmental protection for the European aviation system. The programme aims at collecting and gathering all data that may support the management of safety risks at European level. This includes safety reports (or occurrences), flight data (i.e. data generated by the aircraft via the flight data recorders), surveillance data (air traffic data), weather data - but those are only a few from a much longer list. As for the analysis, the programme’s ultimate goal is to help to ‘know where to look’ and to ‘see it coming’. In other words, it will support the performance-based environment and set up a more predictive system. More specifically, the programme will facilitate better knowledge of where the risks are (safety issue identification), determine the nature of these risks (risk assessment) and verify whether the safety actions are delivering the needed level of safety (performance measurement). It aims to develop the capability to discover vulnerabilities in the system across terabytes of data
	}
} 

\newglossaryentry{Deep learning} {
	name={Deep learning (DL)},
	text={deep learning},
	description={A specific type of machine learning based on the use of large neural networks to learn abstract representations of the input data by composing many layers}
}

\newglossaryentry{Digital twin} {
	name={Digital twin},
	text={digital twin},
	description={ {\sl ``A digital twin is a virtual representation that serves as the real-time digital counterpart of a physical object or process.''}\footnote{\url{https://en.wikipedia.org/wiki/Digital_twin}}}
}

\newglossaryentry{Embodied artificial intelligence (EAI)} {
	name={Embodied artificial intelligence (EAI)},
	description={In EAI, AI algorithms learn through embodied physical interactions with their environments, whether real or simulated}
} 

\newglossaryentry{Epistemology} {
	name=Epistemology,
	description={The study of knowledge and the justification of beliefs}
}

\newglossaryentry{Epistemologic defeaters} {
	name={Epistemologic defeaters},
	description={Conditions or events leading to  the   loss, reduction, or prevention of some positive epistemic status, that is, conditions or events counting {\it against} a belief}
}

\newglossaryentry{Explainable AI} {
	name={Explainable AI},
	description={{\sl `` is artificial intelligence (AI) in which the results of the solution can be understood by humans.''}\footnote{\url{https://en.wikipedia.org/wiki/Explainable_artificial_intelligence}}}
}

\newglossaryentry{Functional safety}{
	name={Functional safety},
	description={is the part of the overall safety of a system or piece of equipment that depends on automatic protection operating correctly in response to its inputs or failure in a predictable manner (fail-safe). The automatic protection system should be designed to properly handle likely human errors, systematic errors, hardware failures and operational/environmental stress.\footnote{definintion adopted verbatim from \url{https://en.wikipedia.org/wiki/Functional_safety}}}
}  

\newglossaryentry{Illocutionary force} {
	name={Illocutionary force},
	description={The intention of the sender in a message exchanged between agents}
}

\newglossaryentry{Impact analysis} {
	name={Impact analysis},
	text={impact analysis},
	description={(also {\bf change impact analysis}) {\sl ``is the analysis of changes within a deployed product or application and their potential consequences''}.\footnote{\url{https://en.wikipedia.org/wiki/Change_impact_analysis}}}
} 

\newglossaryentry{Incident} {
	name=Incident,
	text=incident,
	description={Any unexpected event that does not result in serious losses or injury, but {\it might} have caused an accident. For formally, an incident occurs if a system reaches a hazardous state from which it recovers without entering an accident state before}
}

\newglossaryentry{Inference} {
	name=Inference,
	description={The process of feeding the machine learning model an input and computing its output. See also related definition of ‘Training’}
}

\newglossaryentry{Internet of things (IoT)} {
	name={Internet of things (IoT)},
	description={The network of physical objects that contain embedded technology to communicate and sense or interact with their internal states or the external environment}
}

\newglossaryentry{Machine learning} {
	name={Machine learning (ML)},
	text={machine learning},
	description={Rooted in statistics and mathematical optimisation, machine learning is the ability of computer systems to improve their performance by exposure to data without the need to follow explicitly programmed instructions. [Machine learning is a branch of artificial intelligence]. Machine learning strategies go by three methods \gls{Supervised learning}, \gls{Unsupervised learning} and \gls{Reinforcement learning} }
} 

\newglossaryentry{Supervised learning} {
	name={Supervised learning},
	description={- the process of learning a function that maps an input to an output based on example input-output training samples}
}

\newglossaryentry {Unsupervised learning} {
	name={Unsupervised learning},
	description={- this strategy is used in cases where there is no labelled data set available to learn from. The neural network analyses the data set, and then a cost function tells the neural network how far off target it was. The neural network then adjusts to increase accuracy of the algorithm}
}

\newglossaryentry {Reinforcement learning} {
	name={Reinforcement learning},
	description={In this algorithm, the neural network is reinforced for positive results, and punished for a negative result, forcing the neural network to learn over time}
}

\newglossaryentry{Machine learning model} {
	name={Machine learning model},
	description={A parametrised function that maps inputs to outputs. The parameters are determined during the training process}
}

\newglossaryentry{minimal risk condition} {
	name={minimal risk condition},
	description={Vehicle state in order to reduce the risk of harm, when a given trip cannot be completed}
}

\newglossaryentry{Mode confusion} {
	name={Mode confusion},
	text={mode confusion},
	description={The actual system state differs from what a responsible human (e.g.~driver, pilot) thinks the state is (e.g.~pilot thinks that auto pilot is active while it is actually switched off)}
} 

\newglossaryentry{Model-driven AI} {
	name={Model-driven AI},
	description={Model-driven AI (or symbolic AI), instead, attempts to capture knowledge and derive decisions through explicit representation and rules}
}

\newglossaryentry{Narrow AI} {
	name={Narrow AI},
	description={Artificial intelligence that is focused on one narrow task}
}

\newglossaryentry{Open Services for Lifecycle Collaboration (OSLC)} {
	name={Open Services for Lifecycle Collaboration (OSLC)},
	description={is an open community creating specifications for {\it interactions between tools}. The objective is to facilitate the development of IDEs, including issue tracking, testing, and other services relevant for  the lifecycle of software-based products. In particular, IDEs should become more flexible with the help of OSLC, so that it will become easier to integrated tools of other providers, as long as these tools conform to the data exchange protocols provided by OSLC}
}

\newglossaryentry{Operational safety} {
	name={Operational safety},
	description={means the absence of unreasonable risk under the occurrence of hazards resulting from functional insufficiencies of the intended functionality (e.g. false/missed detection), operational disturbances (e.g. environmental conditions like fog, rain, shadows, sunlight, infrastructure) or by reasonably foreseeable misuse/errors by the driver, passengers and other road users (safety hazards — without system faults).\footnote{definition adopted verbatim from \url{https://www.lawinsider.com/dictionary/operational-safety}}}
}

\newglossaryentry{Performative} {
	name={Performative},
	description={same meaning as \emph{illocutionary force}}
} 

\newglossaryentry{Predictability/determinism} {
	name={Predictability/determinism},
	description={A system is predictable/deterministic if when given identical inputs, produces identical outputs}
}

\newglossaryentry{Rebutting defeater} {
	name={Rebutting defeater},
	text={rebutting defeater},
	description={A defeater (in epistemology) providing evidential support for the opposite thesis of a belief}
} 

\newglossaryentry{Resilience} {
	name=Resilience,
	description={Attribute of systems and applications to ensure high service availability through monitoring and automatic adjustment of redundant or virtualized infrastructure components}
}

\newglossaryentry{Road furniture}{
	name={Road furniture (also street furniture)},
	text={road furniture (also street furniture)},
	description={A collective term for objects and pieces of equipment installed along streets and roads for various purposes. It includes benches, traffic barriers, bollards, post boxes, phone boxes, streetlamps, traffic lights, traffic signs, bus stops, tram stops, taxi stands, public lavatories, fountains, watering troughs, memorials, public sculptures, and waste receptacles}
}

\newglossaryentry{Robustness}{
	name={Robustness},
	text={robustness},
	description={For an input varying in a region of the state space, the system is producing the same outputs}
}

\newglossaryentry{Safety science} {
	name={Safety science},
	description={A broad field that refers to the collective processes, theories, concepts, tools and technologies that support safety management}
}

\newglossaryentry{Safing mission} {
	name={Safing mission},
	description={A behaviour triggered when sudden events increase the risk in an unacceptable way. Theobjective of this behaviour is to transfer the system into a stable safe state  as quickly as possible~\citep{DBLP:journals/itsm/KoopmanW17}}
}

\newglossaryentry{Training} {
	name=Training,
	text=training,
	description={The process of optimising the parameters (weights) of a machine learning model given a data set and a task to achieve on that data set. For example, in supervised learning, the training data consists of input (e.g. an image) / output (e.g. a class label) pairs and the machine learning model ‘learns’ the function that maps the input to the output, by optimising its internal parameters. See also related definition of ‘Inference’}
}

\newglossaryentry{Undercutting defeater} {
	name={Undercutting defeater},
	text={undercutting defeater},
	description={A defeater (in epistemology) removing support for a belief}
}

\newglossaryentry{Variance} {
	name={Variance},
	text=variance,
	description={An error from sensitivity to small fluctuations in the training set. High variance can cause an algorithm to model the random noise in the training data, rather than the intended outputs (=overfitting)}
}

\newglossaryentry{Vulnerable Road User (VRU)} {
	name={Vulnerable Road User (VRU)},
	description={A road user who is not occupying a vehicle such as a passenger car, a public transit vehicle, or a train}
}

\newglossaryentry{Vehicle to everything (V2X) communication} {
	name={Vehicle to everything (V2X) communication},
	description={Communication between a (potentially autonomous) vehicle and {\sl ``any entity that may affect, or may be affected by, the vehicle.''}\footnote{\url{https://en.wikipedia.org/wiki/Vehicle-to-everything}}}
}


